Asymptotic Classification Error for Heavy-Tailed Renewal Processes

Despite the widespread occurrence of classification problems and the increasing collection of point process data across many disciplines, study of error probability for point process classification only emerged very recently. Here, we consider classification of renewal processes. We obtain asymptotic expressions for the Bhattacharyya bound on misclassification error probabilities for heavy-tailed renewal processes.

==> ap-pf-v3.tex <==
%%%%%%++++++++++++++++++++++++III.C
\appendix
\renewcommand{\theequation}{A.\arabic{equation}}
We prove Theorem \ref{Bhvy}. 
Under A1 and by Lemma 1, we have
\eqn{
\label{Ga}
\Gwt(x) \sim x^{-\rho}L(x).
}
The following Results 1-3 prove Theorem 3 in three steps, based on the value of $\rho$. 

%%%%%
\subsubsection{Step 1: $0<\rho<1$}
The asymptotic relation (\ref{Ba}) is 
a direct application of the KT theorem. 

%%%+++++++++++++++++++++++++++++++Result 1
{\it Result 1:} 
The relation (\ref{Ba}) holds when $0<\rho<1$. 


{\it Proof. }
For $0<\rho<1$, the relation (\ref{Ga}) and Theorem \ref{TA} give
$
\Gwt(x)\sim x^{-\rho}L(x)\Ra \bGwt(s) \sim\frac{\Gam(1-\rho)}{s^{1-\rho}}L(\frac1s).
$ 
Then, note that $\bpwt(0) = \intoi \pwt(x)dx = \cwt$. We have 
$
\bar B(s) = \frac{\bGwt(s)}{1-\bpwt(s)} \sim \frac{\Gam(1-\rho)}{(1-\cwt)s^{1-\rho}}L(\frac1s),0<\rho<1, 
$
as $\stoo$. 
Now use Theorem \ref{TA} again to get (\ref{Ba}). 
\hfill$\square$


%%%%%
\subsubsection{Step 2: $\rho=1$}
This case is not straightforward 
since (a) and (b) in Theorem \ref{TA} do not imply each other when $\rho=1$. 
Thus, instead, we analyze the LT of $P(T)=TB(T)$. 
The LT exists on $s\in(0,\infty)$ since $P(T)$ is bounded by a polynomial with finite power. 
We need the following lemmas.


%%%+++++++++++++++++++++++222222222222222222222bbbb
{\it Lemma A: } Let $L(x)$ be slowly varying and locally bounded on $[a,\infty),a>0$ 
and $S(x)\sim x^{-1}L(x)$ at $\infty$. Then, 
$U(x) = \intox S(u)du \sim L_*(x)$ at $\infty$, 
where $L_*(x)=\int_a^x u^{-1}L(u)du$ is slowly varying. 

{\it Proof.} 
This is a slight generalization of \cite[Proposition 1.5.9a]{Bing87}. 
The proof is simple and thus omitted.
\hfill$\square$


%%%+++++++++++++++++++++++BBBBBBBBBBBBBBBBBB
{\it Lemma B: } $\pwt(x)\leq\qwt(x)${, 
where $\qwt$ is the density function whose survivor function is $\Gwt$ and is given in (\ref{q12})}. 

{\it Proof.}
Use the hazard relations (\ref{hr}) %
to find 
$\pwt(x)=\sqrt{h_1(x)h_2(x)}\Gwt(x)\leq \frac{h_1(x)+h_2(x)}{2}\Gwt(x) = \qwt(x)$.\hfill$\square$



%%%+++++++++++++++++++++++++++++++Result 2 
{\it Result 2: }
The relation (\ref{Ba}) holds when $\rho=1$. 


{\it Proof.}
Introduce $P(T) = TB(T)$. 
Then its LT
$
\bar P(s) = \intoi e^{-sT}TB(T)dT = -\bar B'(s) 
	= \frac{-\bGwt'(s)}{1-\bpwt(s)} + \frac{\bpwt'(s)\bGwt(s)}{(1-\bpwt(s))^2}, s>0
$. 
We have $\bpwt(0)=\cwt$. So we examine $\bGwt'(s),\bpwt'(s)$ and $\bGwt(s)$. 
First, $-\bGwt'(s)$ is the LT of $x\Gwt(x)$ and 
$x\Gwt(x)\sim L(x)$, as $\xtoi\Ra -\bGwt'(s)\sim \frac1sL(\frac1s)$, as $\stoo$. 
Now use Lemma A and Theorem \ref{TA} to get
$U(x) = \intox \Gwt(u)du \sim L_*(x){=\intox u^{-1}L(u)du}$, as $\xtoi\Ra\bGwt(s)\sim \bar L_*(\frac1s)$, as $\stoo$, 
where $\Ls(x)$ is slowly varying due to Lemma A{ and $\bar L_\ast(s)$ is the LT of $\Ls(x)$}. 
Then, due to Lemma B, we have for real $s>0$, 
$-\bpwt'(s) = \intoi e^{-sx}x\pwt(x)dx
	\leq \intoi e^{-sx}x\qwt(x)dx 
	= \intoi e^{-sx}xd(-\Gwt(x))
	= 0 + \intoi\Gwt(x)(e^{-sx}-sxe^{-sx})dx
	= \bGwt(s) + s\bGwt'(s)$.  
This indicates that for $s>0$, 
\eq{
\frac{-\bpwt'(s)\bGwt(s)}{\frac1sL\bra{1/s}}&\leq\frac{[\bGwt(s)+s\bGwt'(s)]\bGwt(s)}{\frac1sL\bra{1/s}}\sim {s\hat L(1/s),}%
}
{where $\hat L(\wos)=\frac{L_*\bra{1/s}\sqbra{L_*\bra{1/s}-L\bra{1/s}}}{L\bra{1/s}}$ 
is slowly varying by Lemma 1, and we conclude $s\hat L(1/s)\to0$ also by Lemma 1.}

We thus find that $-\bGwt'(s)$ dominates $\bar P(s)$, so that 
$\bar P(s)\sim\frac{1}{1-\cwt}\frac1sL(\frac1s)$, as $\stoo\Ra P(T)\sim\frac{1}{1-\cwt}L(T)$, as $\Ttoi\Ra B(T) \sim\frac{1}{1-\cwt}T^{-1}L(T)$, as $\Ttoi$,
as needed.
\hfill$\square$


%%%%%
\subsubsection{Step 3: $\rho>1$} 
The KT theorem does not cover this case. 
We now need to analyze the LT of $P_m(T) = T^mB(T)$,  
where the integer $m$ satisfies
\eq{
x^m\Gwt(x) \sim x^{-\beta}L(x),\quad 0<\beta=\rho-m\leq1.
}
The LT also exists by the same arguments above. 
In this case, we need more results about the non-dominating LT terms. 
Let $f^{(n)}$ be the $n$-th derivative of $f$. 
The following lemmas hold. 

%%%+++++++++++++++++++++++CCCCCCCCCCCCCCCCC
{\it Lemma C: } 
For all integers $n<m$, $(-1)^n\bGwt^{(n)}(0)=\intoi x^n\Gwt(x)dx<\infty$. (cf. \cite[Proposition 1.5.10]{Bing87})


%%%+++++++++++++++++++++++DDDDDDDDDDDDDDDD
{\it Lemma D: } 
For all integers $n\leq m$, $(-1)^n\bpwt^{(n)}(0)=\intoi x^n\pwt(x)dx<\infty$.


{\it Proof.}
{It suffices to consider
$\intoi x^m\pwt(x)dx\leq\intoi x^m\qwt(x)dx
= \intoi x^md(-\Gwt(x))
= -x^m\Gwt(x)\vert_0^\infty + m\intoi\Gwt(x)x^{m-1}dx
= m(-1)^{m-1}\bGwt^{(m-1)}(0)<\infty$.
The inequalities follow from Lemma B and Lemma C.} 
\hfill$\square$


%%%+++++++++++++++++++++++++++++++Result 3
{\it Result 3: }
The relation (\ref{Ba}) holds when $\rho>1$.


{\it Proof.}
We need to discuss two cases. 

First, for $0<\beta<1$, 
let $P_m(T) = T^mB(T)$. 
Its LT has the term
$\frac{(-1)^m\bGwt^{(m)}(s)}{1-\bpwt(s)}$, 
and all other terms have finite limits as $\stoo$ due to Lemma C and Lemma D. 
Then following the same as in the proof of Result 1 gives the quoted result. 

Now consider $\beta=1$ and $P_{m+1}(T) = T^{m+1}B(T)$. 
We need to examine its LT terms with 
$\bGwt^{(m)}, \bGwt^{(m+1)}$ and $\bpwt^{(m+1)}$, 
which are possibly infinite as $\stoo$. 
The following is parallel to the proof of Result 2. 
Using integral by parts and Lemma B, we get, for $s>0$, 
$(-1)^n\bpwt^{(n)}(s) \leq \bGwt(s) + (-1)^{n-1}s\bGwt^{(n)}(s)$. 
We also find that $\bGwt^{(m)}(s)$ is only slowly varying but 
$(-1)^{m+1}\bGwt^{(m+1)}(s)\sim \frac1sL(\frac1s)$ is regularly varying. 
Then, we find that $\bpwt^{(m+1)}(s)$ is only slowly varying. 
However, the only term containing $\bGwt^{(m+1)}$ is 
$\frac{(-1)^{m+1}\bGwt^{(m+1)}(s)}{1-\bpwt(s)}$, 
so it still dominates. The result then also follows easily.
\hfill$\square$
%

